If Loud Aliens Explain Human Earliness, Quiet Aliens Are Also Rare

If life on Earth had to achieve n 'hard steps' to reach humanity's level, then the chance of this event rose as time to the n-th power. Integrating this over habitable star formation and planet lifetime distributions predicts >99% of advanced life appears after today, unless n<3 and max planet duration <50Gyr. That is, we seem early. We offer this explanation: a deadline is set by 'loud' aliens who are born according to a hard steps power law, expand at a common rate, change their volumes' appearances, and prevent advanced life like us from appearing in their volumes. 'Quiet' aliens, in contrast, are much harder to see. We fit this three-parameter model of loud aliens to data: 1) birth power from the number of hard steps seen in Earth history, 2) birth constant by assuming a inform distribution over our rank among loud alien birth dates, and 3) expansion speed from our not seeing alien volumes in our sky. We estimate that loud alien civilizations now control 40-50% of universe volume, each will later control ~10^5 - 3x10^7 galaxies, and we could meet them in ~200Myr - 2Gyr. If loud aliens arise from quiet ones, a depressingly low transition chance (~10^-4) is required to expect that even one other quiet alien civilization has ever been active in our galaxy. Which seems bad news for SETI. But perhaps alien volume appearances are subtle, and their expansion speed lower, in which case we predict many long circular arcs to find in our sky.

==> newbibs.tex <==
*** \textbf{References to add to References Section: }

Westby, Tom, and Christopher Conselice (2020) “The Astrobiological Copernican Weak and Strong Limits for Intelligent Life” The Astrophysical Journal, 896(1):58 June https://doi.org/10.3847/1538-4357/ab8225 

Lingam, Manasvi, Idan Ginsburg, and Abraham Loeb (2020) “Prospects for Life on Temperate Planets around Brown Dwarfs” The Astrophysical Journal, Volume 888(2): 102, January.

Zeng, Li, Stein B. Jacobsen, Eugenia Hyung, Andrew Vanderburg, Mercedes Lopez-Morales, Dimitar D. Sasselov, Juan Perez-Mercader, Michail I. Petaev, David W. Latham, Raphaëlle D. Haywood, Thomas K. R. Mattson (2018) "Planet Size Distribution from the Kepler Mission and its Implications for Planet Formation" https://arxiv.org/abs/1806.05909

Hart, Michael (1975) “Explanation for the Absence of Extraterrestrials on Earth” 
Quarterly Journal of the Royal Astronomical Society, 16:128

Benford, James, Gregory Benford, and Dominic Benford (2010) "Messaging with Cost-Optimized Interstellar Beacons" Astrobiology 10(5):475-490. June, http://doi.org/10.1089/ast.2009.0393

Lacki, Brian (2020) "Lens Flare: Magnified X-Ray Binaries as Passive Beacons in SETI" https://arxiv.org/abs/2002.00128

 Balbi, Amedeo, Milan M. Ćirković (2021) "Longevity is the key factor in the search for technosignatures" https://arxiv.org/abs/2103.02923

Wandel, Amri, Joe Gale (2020) “The bio-habitable zone and atmospheric properties for planets of red dwarfs” International Journal of Astrobiology 19(2):126-135, https://doi.org/10.1017/S1473550419000235

Stevenson, David (2019a) “Niche amplitude, tidal-locking and Fermi's Paradox” International Journal of Astrobiology 18(4):377 - 383, August https://doi.org/10.1017/S1473550418000253

Lingam, Manasvi, Abraham Loeb (2019b) “Brown Dwarf Atmospheres as the Potentially Most Detectable and Abundant Sites for Life” The Astrophysical Journal 883(2):143 September 

Lingam, Manasvi, Abraham Loeb (2019a) “Subsurface exolife” International Journal of Astrobiology 18(2):112-141, April https://doi.org/10.1017/S1473550418000083

Ben Pearce, Andrew Tupper, Ralph Pudritz, and Paul Higgs (2018) “Constraining the Time Interval for the Origin of Life on Earth” Astrobiology 18(3):343-364, March.  https://doi.org/10.1089/ast.2017.1674

Ozaki, Kazuma, Christopher Reinhard (2021) “The future lifespan of Earth’s oxygenated atmosphere.” Nature Geoscience https://doi.org/10.1038/s41561-021-00693-5

Forgan, Duncan, Pratika Dayal, Charles Cockell, and Noam Libeskind (2017) “Evaluating galactic habitability using high-resolution cosmological simulations of galaxy formation” International Journal of Astrobiology 16 (1): 60–73 doi:10.1017/S1473550415000518 

Mason, Paul, Jorge Zuluaga, Pablo A. Cuartas-Restrepo, and Joni M. Clark (2015) “Circumbinary habitability niches” International Journal of Astrobiology 14(3):391–400 doi:10.1017/S1473550414000342 

Martin, Andrew, Andrew McMinn (2018) “Sea ice, extremophiles and life on extra-terrestrial ocean worlds” International Journal of Astrobiology , 17(1):1-16, January, https://doi.org/10.1017/S1473550416000483

Simpson, Fergus (2017) “The longevity of habitable planets and the development of intelligent life” \textit{International Journal of Astrobiology} 16(3):266 - 270, July https://doi.org/10.1017/S1473550416000306

Gale, Joseph, Amri Wandel (2017) "The potential of planets orbiting red dwarf stars to support oxygenic photosynthesis and complex life" International Journal of Astrobiology 16 (1): 1–9 doi:10.1017/S1473550415000440 

Peter Behroozi, Molly Peeples (2015) "On the history and future of cosmic planet formation" \textit{Monthly Notices of the Royal Astronomical Society} 454(2):1811–1817, December, https://doi-org.mutex.gmu.edu/10.1093/mnras/stv1817

Sloan, David, Rafael Batista, Abraham Loeb (2017) “The Resilience of Life to Astrophysical Events” \textit{Scientific Reports} 7:5419, DOI:10.1038/s41598-017-05796-x

Loeb, Abraham, Rafael Batista, and David Sloan (2016) “Relative likelihood for life as a function of cosmic time”
\textit{Journal of Cosmology and Astroparticle Physics}, August 18. https://iopscience.iop.org/article/10.1088/1475-7516/2016/08/040

Haqq-Misra, Jacob, Ravi Kumar Kopparapu and Eric T. Wolf (2018) “Why do we find ourselves around a yellow star instead of a red star?” \textit{International Journal of Astrobiology} 17 (1): 77–86 doi:10.1017/S1473550417000118 

Lingam, Manasvi, and Abraham Loeb (2018) “Is life most likely around Sun-like stars?” \textit{Journal of Cosmology and Astroparticle Physics}, May. https://doi.org/10.1088/1475-7516/2018/05/020

Lingam, Manasvi and Abraham Loeb (2019) “Role of stellar physics in regulating the critical steps for life” International \textit{Journal of Astrobiology }18(6):527 - 546, December  https://doi.org/10.1017/S1473550419000016

Waltham, David (2017) “Star Masses and Star-Planet Distances for Earth-like Habitability” \textit{Astrobiology} 17(1)  DOI: 10.1089/ast.2016.1518

Nunney, Leonard (2015) “Commentary: The multistage model of carcinogenesis, Peto’s paradox and evolution” International \textit{Journal of Epidemiology}, 649–653 doi:10.1093/ije/dyv201 December

Olson, S. Jay (2015) “Homogeneous cosmology with aggressively expanding civilizations” 
\textit{Classical and Quantum Gravity}, 32(21):215025
DOI: 10.1088/0264-9381/32/21/215025

Olson, S. Jay (2016) “On the visible size and geometry of aggressively expanding civilizations at cosmological distances”
\textit{Journal of Cosmology and Astroparticle Physics}, April
DOI: 10.1088/1475-7516/2016/04/021

Olson, S. Jay (2017) “Estimates for the number of visible galaxy-spanning civilizations and the cosmological expansion of life”
\textit{International Journal of Astrobiology} , 16(2):176-184, April. 
DOI: https://doi.org/10.1017/S1473550416000082

Olson, S. Jay (2018a) “Long-term implications of observing an expanding cosmological civilization”
\textit{International Journal of Astrobiology} , 17(1): 87-95, January.
 https://doi.org/10.1017/S147355041700012X

Olson, S. Jay (2018b) “Expanding cosmological civilizations on the back of an envelope” arXiv:1805.06329 

Olson, S. Jay (2020) “On the Likelihood of Observing Extragalactic Civilizations: Predictions from the Self-Indication Assumption” 
arXiv:2002.08194

Wolfram Research, Inc., Mathematica, Version 12.2, Champaign, IL (2020).  *** This was supposed to be in prior draft, and somehow got dropped ***

McCabe, Michael and Holly Lucas (2010) “On the origin and evolution of life in the galaxy”
\textit{International Journal of Astrobiology} 9(4):217 - 226, October. 
https://doi.org/10.1017/S1473550410000340   *** this is a change to an existing reference ***
